On The Distribution of Penultimate Activations of Classification Networks

This paper studies probability distributions of penultimate activations of classification networks. We show that, when a classification network is trained with the cross-entropy loss, its final classification layer forms a Generative-Discriminative pair with a generative classifier based on a specific distribution of penultimate activations. More importantly, the distribution is parameterized by the weights of the final fully-connected layer, and can be considered as a generative model that synthesizes the penultimate activations without feeding input data. We empirically demonstrate that this generative model enables stable knowledge distillation in the presence of domain shift, and can transfer knowledge from a classifier to variational autoencoders and generative adversarial networks for class-conditional image generation.

==> figs/hvae.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figs/hvae/hvae_0698.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figs/hvae/hvae_1723.png}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figs/hvae/hvae_5182.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figs/hvae/hvae_9716.png}
    \end{subfigure}
    \caption{
        Visualization of the latent space of HVAE-L.
        We interpolate between class centers of randomly selected labels.
    }
    \label{fig:hvae}
\end{figure}

==> figs/sunflower_add.tex <==
%% Additional sunflower plots. Appears in appendix.
\begin{figure}[ht]
    \label{fig:mnist_app}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/2d_teacher1}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/2d_teacher2}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/2d_teacher4}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/2d_teacher8}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/2d_teacher30} \\
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/2d_teacher1}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/2d_teacher2}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/2d_teacher4}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/2d_teacher8}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/2d_teacher30} \\
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/2d_teacher1}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/2d_teacher2}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/2d_teacher4}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/2d_teacher8}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/2d_teacher30} \\
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/2d_teacher1}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/2d_teacher2}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/2d_teacher4}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/2d_teacher8}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/2d_teacher30} \\
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/polar_teacher1}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/polar_teacher2}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/polar_teacher4}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/polar_teacher8}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run0/polar_teacher30} \\
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/polar_teacher1}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/polar_teacher2}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/polar_teacher4}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/polar_teacher8}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run1/polar_teacher30} \\
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/polar_teacher1}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/polar_teacher2}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/polar_teacher4}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/polar_teacher8}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run2/polar_teacher30} \\
    \hspace{25pt}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/polar_teacher1}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/polar_teacher2}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/polar_teacher4}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/polar_teacher8}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/run3/polar_teacher30}
    \centering\includegraphics[height=.16\columnwidth]{figs/sunflower/lgnd_only} \\
\caption{
    Additional runs of the $2$-dimensional MNIST experiment.
    We also show kernel density estimates of unnormalized activations.
    \shk{do not explain contents of a figure in this way. }
}
\end{figure}

==> figs/sunflower_kd.tex <==
% !TEX root = ../main.tex

% \setlength{\intextsep}{0pt}
% \begin{wrapfigure}{r}{0.42\linewidth}
% \begin{center}
%     \centering\includegraphics[height=.19\columnwidth]{figs/sunflower/2d_teacher30}
%     \centering\includegraphics[height=.19\columnwidth]{figs/sunflower/2d_student30} \\
%     \centering\includegraphics[height=.19\columnwidth]{figs/sunflower/polar_teacher30}
%     \centering\includegraphics[height=.19\columnwidth]{figs/sunflower/polar_student30_lgnd}
% \end{center}
% \caption{
%     Distillation from teacher (left) to student (right).
%     \lyh{TODO}
% }
% \label{fig:sunflower}
% \end{wrapfigure}

% \vspace{5mm}
% \includegraphics[height=0.45\linewidth]{figs/sunflower/2d_teacher30}
% \includegraphics[height=0.45\linewidth]{figs/sunflower/2d_student30}
% \includegraphics[height=0.45\linewidth]{figs/sunflower/2d_student30}
\begin{figure}
\centering 
\begin{subfigure}[t]{.29\linewidth}
    \includegraphics[width=\linewidth]{figs/sunflower_kd/polar_base30.pdf}
\caption{Teacher} \end{subfigure} 
\begin{subfigure}[t]{.29\linewidth}
    \includegraphics[width=\linewidth]{figs/sunflower_kd/polar_kd30.pdf}
\caption{Student (KD)} \end{subfigure}
\begin{subfigure}[t]{.29\linewidth}
    \includegraphics[width=\linewidth]{figs/sunflower_kd/polar_ckd30.pdf}
\caption{Student (CKD)} \end{subfigure}
\includegraphics[height=0.29\linewidth]{figs/sunflower/lgnd_only.pdf}

\caption{
    Visualization of penultimate activations and their vMF distributions of teacher and student networks on the MNIST dataset.
    $\na$ of datapoints are represented by dots and vMF distributions $q(\na|i)$ are drawn by solid lines.
}
\label{fig:sunflower_kd}
% \vspace{5mm}
\end{figure}






















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NOT USED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
% \vspace{5mm}
\begin{figure}
\centering 
\begin{subfigure}[t]{.43\linewidth}
    % \includegraphics[height=0.45\linewidth]{figs/sunflower/2d_teacher30}
    \includegraphics[width=\linewidth]{figs/sunflower/polar_teacher30}
\caption{Teacher network} \end{subfigure} 
\hfill
\begin{subfigure}[t]{.43\linewidth}
    % \includegraphics[height=0.45\linewidth]{figs/sunflower/2d_student30}
    \includegraphics[width=\linewidth]{figs/sunflower/polar_student30}
\caption{Student network trained with CKD} \end{subfigure}
\includegraphics[width=0.09\linewidth]{figs/sunflower/lgnd_only.pdf}

\caption{
    Visualization of penultimate activations and their vMF distributions on the MNIST dataset. 
    For both of the teacher and student, ({\bf left}) kernel density estimates of $\ba$, ({\bf right}) distributions of $\na$ represented by dots and vMF distributions $q(\na|i)$ drawn by solid lines.
}
\label{fig:sunflower_kd}
% \vspace{5mm}
\end{figure}


\begin{figure}[h!]
    \centering\includegraphics[height=.22\columnwidth]{figs/sunflower/2d_teacher30}
    \centering\includegraphics[height=.22\columnwidth]{figs/sunflower/polar_teacher30} \quad
    \centering\includegraphics[height=.22\columnwidth]{figs/sunflower/2d_student30} 
    \centering\includegraphics[height=.22\columnwidth]{figs/sunflower/polar_student30_lgnd}
\caption{
Penultimate activations and their vMF distributions of the teacher network ({\bf left}) and those of the student network trained with CKD ({\bf right}).
}
\label{fig:sunflower_kd}
\end{figure}


\vspace{5mm}
\begin{figure}[h!]
    \centering \begin{subfigure}[t]{.22\linewidth}
    \includegraphics[height=\linewidth]{figs/sunflower/2d_teacher30}
    \caption{} \end{subfigure}
    \centering \begin{subfigure}[t]{.22\linewidth}
    \includegraphics[height=\linewidth]{figs/sunflower/polar_teacher30}
    \caption{} \end{subfigure} 
    \quad
    \centering \begin{subfigure}[t]{.22\linewidth}
    \includegraphics[height=\linewidth]{figs/sunflower/2d_student30}
    \caption{} \end{subfigure}
    \centering \begin{subfigure}[t]{.22\linewidth}
    \includegraphics[height=\linewidth]{figs/sunflower/polar_student30_lgnd}
    \caption{} \end{subfigure}
\caption{
Visualization of penultimate activations and their vMF distributions on the MNIST dataset. (a) $\ba$ of $T$. (b) $\na$ and vMF distributions of $T$. (c) $\ba$ of $S$. (d) $\na$ and vMF distributions of $S$.
}
\label{fig:sunflower_kd}
\vspace{5mm}
\end{figure}


\begin{figure}
    \centering \begin{subfigure}[t]{.46\linewidth}
    \includegraphics[height=0.45\linewidth]{figs/sunflower/2d_teacher30}
    \includegraphics[height=0.45\linewidth]{figs/sunflower/polar_teacher30}
    \caption{Teacher network} \end{subfigure} 
    \quad
    \centering \begin{subfigure}[t]{.46\linewidth}
    \includegraphics[height=0.45\linewidth]{figs/sunflower/2d_student30}
    \includegraphics[height=0.45\linewidth]{figs/sunflower/polar_student30_lgnd}
    \caption{Student network trained with CKD} \end{subfigure}
\caption{
Visualization of penultimate activations and their vMF distributions on the MNIST dataset. For both of the teacher and student, ({\bf left}) kernel density estimates of $\ba$, ({\bf right}) distributions of $\na$ represented by dots and vMF distributions $q(\na|i)$ drawn by solid lines.
}
\label{fig:sunflower_kd}
% \vspace{5mm}
\end{figure}
\fi 


==> preamble.tex <==
\usepackage{subcaption}
\usepackage{ragged2e}
\usepackage{commath} % abs, norm
\usepackage{xspace}
\usepackage{booktabs}
\usepackage[up,bf,raggedright]{titlesec}
\usepackage{siunitx,etoolbox}
\usepackage{algorithm,algorithmic} % algorithm env
\usepackage{multirow}
\usepackage{xpatch}
\xpretocmd{\eqref}{Eq.~}{}{}

\usepackage{amsthm, mathtools}
\newtheorem{theorem}{{Theorem}}
\newtheorem{lemma}{{Lemma}}

% siunitx setup. used in tables
\sisetup{
    round-mode=places, 
    round-precision=2, 
    table-align-uncertainty=true, 
    separate-uncertainty=true,
    detect-weight, 
    mode=text
}

\usepackage[dvipsnames]{xcolor}
% 0
% \hypersetup{draft}


% for highlighting in algorithm
\usepackage{tikz}
\usetikzlibrary{fit,calc}
\newcommand*{\tikzmk}[1]{\tikz[remember picture,overlay] \node (#1) {};\ignorespaces}
\newcommand{\boxit}[1]{\tikz[remember picture,overlay]{\node[yshift=2pt,fill=#1,opacity=.10,fit={(A)(B)}] {};}\ignorespaces}


\usepackage[capitalize,nameinlink,noabbrev]{cleveref} %cref, import last


% Use \BF to make a table cell bold.
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
\newrobustcmd{\BF}{\bfseries}

\newcommand{\todo}[1]{\textcolor{red}{(\textbf{TODO}: #1)}}
\newcommand{\shk}[1]{{\color{red} (shk: #1)}}
\newcommand{\lyh}[1]{{\color{blue} (lyh: #1)}}
\newcommand{\mks}[1]{{\color{green} (mks: #1)}}
\newcommand{\new}[1]{{\color{red} (NEW: #1)}}

\def\ie{\emph{i.e.}}
\def\eg{\emph{e.g.}}
\def\etal{\emph{et al.}}
\def\wrt{\emph{w.r.t.}}

\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{#1\;\delimsize|\delimsize|\;#2}
\newcommand{\kld}[2]{\ensuremath{D_{KL}\infdivx{#1}{#2}}\xspace}

\newcommand{\na}{\overline{\ba}}
\newcommand{\nw}{\overline{\bw}}



==> tables/kd_algs.tex <==
\newcommand{\hilight}[1]{\tikzmk{A}#1\tikzmk{B}\boxit{red}}

\vspace{-5pt}\noindent%
\begin{minipage}[t!]{0.48\textwidth}
\begin{algorithm}[H] \begin{algorithmic}[1]
\caption{KD \citep{hinton_distilling_2015}}
\label{alg:kd}
    \REQUIRE teacher network $\bx \mapsto p_T(y|\bx)$
    \REQUIRE student network $\bx \mapsto p_S(y|\bx)$
    \WHILE{not converged}
        \STATE $\bx, i \sim p(\bx, i)$
        \STATE \hilight{$p_T \Leftarrow p_T(y|\bx)$}
        \STATE $p_S \Leftarrow p_S(y|\bx)$
        \STATE $\mathcal{L}_\textrm{KD} \Leftarrow - p_T \cdot \log p_S$
    \ENDWHILE
\end{algorithmic} \end{algorithm}
\end{minipage}%
\vspace{5pt}
\begin{minipage}[t!]{0.48\textwidth}
\begin{algorithm}[H] \begin{algorithmic}[1]
\caption{Class-wise KD (ours)}
\label{alg:ckd}
    \REQUIRE teacher network $\bx \mapsto p_T(y|\bx)$
    \REQUIRE student network $\bx \mapsto p_S(y|\bx)$
    \STATE \hilight{
        $p_T(y|i) \Leftarrow \frac{1}{N} \sum_{j=1}^N p_T(y|\na_j)$}
    \WHILE{not converged}
        \STATE $\bx, i \sim p(\bx, i)$
        \STATE \hilight{$p_T \Leftarrow p_T(y|i)$}
        \STATE $p_S \Leftarrow p_S(y|\bx)$
        \STATE $\mathcal{L}_\textrm{CKD} \Leftarrow - p_T \cdot \log p_S$
    \ENDWHILE
\end{algorithmic} \end{algorithm}
\end{minipage}

==> tables/kd_algs_backup.tex <==
\newcommand{\hilight}[1]{\setlength{\fboxsep}{0pt}\colorbox{red!10}{#1}}
\vspace{-5pt}
% \noindent\begin{minipage}[t]{0.49\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\caption{KD \citep{hinton_distilling_2015}}
\label{alg:kd}
    \Require teacher network $\bx \mapsto p_T(y|\bx)$
    \Require student network $\bx \mapsto p_S(y|\bx)$
    \While{not converged}
        \State $\bx, i \sim p(\bx, i)$
        \State \hilight{$p_T \Leftarrow p_T(y|\bx)$}
        \State $p_S \Leftarrow p_S(y|\bx)$
        \State $\mathcal{L}_\textrm{KD} \Leftarrow - p_T \cdot \log p_S$
    \EndWhile
\end{algorithmic}
\end{algorithm}
% \end{minipage}\hspace{0.02\textwidth}%
% \begin{minipage}[t]{0.49\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\caption{Class-wise KD (ours)}
\label{alg:ckd}
    \Require teacher network $\bx \mapsto p_T(y|\bx)$
    \Require student network $\bx \mapsto p_S(y|\bx)$
    \State \hilight{$p_T(y|i) \Leftarrow \frac{1}{N} \sum_{j=1}^N p_T(y|\na_j)$}
    \While{not converged}
        \State $\bx, i \sim p(\bx, i)$
        \State \hilight{$p_T \Leftarrow p_T(y|i)$}
        \State $p_S \Leftarrow p_S(y|\bx)$
        \State $\mathcal{L}_\textrm{CKD} \Leftarrow - p_T \cdot \log p_S$
    \EndWhile
\end{algorithmic}
\end{algorithm}
% \end{minipage}
